A neural prosody encoder for end-ro-end dialogue act classification

Dialogue act classification (DAC) is a critical task for spoken language understanding in dialogue systems. Prosodic features such as energy and pitch have been shown to be useful for DAC. Despite their importance, little research has explored neural approaches to integrate prosodic features into end-to-end (E2E) DAC models which infer dialogue acts directly from audio signals. In this work, we propose an E2E neural architecture that takes into account the need for characterizing prosodic phenomena co-occurring at different levels inside an utterance. A novel part of this architecture is a learnable gating mechanism that assesses the importance of prosodic features and selectively retains core information necessary for E2E DAC. Our proposed model improves DAC accuracy by 1.07% absolute across three publicly available benchmark datasets.

==> problem_definition.tex <==

\newcommand{\dialoglabels}{\{y^\text{diag.}\}}

\newcommand{\pitch}{\boldsymbol{c}}
\newcommand{\energy}{\boldsymbol{e}}
\newcommand{\prosodyframe}{\boldsymbol{p}}
\newcommand{\prosodylist}{P}
\newcommand{\prosodylistextend}{\prosodylist = \{(\energy_1, \pitch_1),...,(\energy_t, \pitch_t)\}}


\newcommand{\audioframe}{\boldsymbol{x}}
\newcommand{\audioframelist}{X=\{\audioframe_1, \audioframe_2, ..., \audioframe_t\}}

\newcommand{\lfbe}{\ell}
\newcommand{\lfbelist}{L=\{\lfbe_1, \lfbe_2, ..., \lfbe_t\}}

\newcommand{\localgate}{\beta}
\newcommand{\globalgate}{\gamma}
\newcommand{\globalprosodiclistname}{V}
\newcommand{\globalprosodic}{\boldsymbol{v}}

\newcommand{\acoustic}{\boldsymbol{a}}
\newcommand{\acousticlistname}{A}
\newcommand{\acousticlist}{\acousticlistname=\{\acoustic_1, \acoustic_2, ..., \acoustic_t\}}

\newcommand{\lstmhidden}{\boldsymbol{h}}
\newcommand{\lstmhiddenlistname}{H}
\newcommand{\lstmhiddenlist}{\lstmhiddenlistname=\{\lstmhidden_1^{(n)}, \lstmhidden_2^{(n)}, ..., \lstmhidden_t^{(n)}\}}

\newcommand{\similaritymatrix}{A^{(s)}}
\newcommand{\dissimilaritymatrix}{A^{(d)}}

\newcommand{\globalgatematrix}{G}

\newcommand{\globalfusion}{F}


% we need to define the problem of dialogue act detection.


We formulate the problem of E2E DAC tasks as follows: 
% In the E2E DAC setting,  to the VA system 
The input is a sequence of raw audio with $t$ time frames, 
%Each audio input extends a growing list of audio frames 
$\audioframelist$. Each $x_t$ is converted to the logarithm of filter bank energy (LFBE) features 
$\lfbelist$ and prosodic acoustic features $\prosodylist = \{(\energy_1, \pitch_1),...,(\energy_t, \pitch_t)\}$,
where $\energy_i \in \mathcal{R}^{|\energy_i|}$ and $\pitch_i \in \mathcal{R}^{|\pitch_i|}$ denote energy and pitch features, respectively. 
Our goal is to correctly classifies DAs for each audio input $X$, namely $\dialoglabels$. 


